Allocation Problems in Ride-Sharing Platforms: Online Matching with Offline Reusable Resources

Bipartite matching markets pair agents on one side of a market with agents, items, or contracts on the opposing side. Prior work addresses online bipartite matching markets, where agents arrive over time and are dynamically matched to a known set of disposable resources. In this paper, we propose a new model, Online Matching with (offline) Reusable Resources under Known Adversarial Distributions (OM-RR-KAD), in which resources on the offline side are reusable instead of disposable; that is, once matched, resources become available again at some point in the future. We show that our model is tractable by presenting an LP-based adaptive algorithm that achieves an online competitive ratio of 1/2 - eps for any given eps greater than 0. We also show that no non-adaptive algorithm can achieve a ratio of 1/2 + o(1) based on the same benchmark LP. Through a data-driven analysis on a massive openly-available dataset, we show our model is robust enough to capture the application of taxi dispatching services and ride-sharing systems. We also present heuristics that perform well in practice.

==> 2_related.tex <==
% !TEX root = 0-17-NIPS.tex

\subsection{Other Related Work}\label{sec:intro-related}



In addition to the arrival assumptions of KIID and KAD, there are several other important, well-studied variants of online matching problems. Under \emph{adversarial ordering}, an adversary can arrange the arrival order of all items in an arbitrary way (e.g., online matching~\cite{kvv,sun2016near} and AdWords~\cite{buchbinder2007online,mehta2007adwords}). 
Under a \emph{random arrival order}, all items arrive in a random permutation order (e.g., online matching~\cite{mahdian2011online} and AdWords~\cite{goel2008online}). Finally, under \emph{unknown distributions}, in each round, an item is sampled from a fixed but unknown distribution. (e.g.,~\cite{devanur2011near}). For each of the above categories, we list only a few examples considered under that setting. For a more complete list, please refer to the book by~\citet{mehta2012online}.

%Even though our model is directly inspired  from lots of applicaitons related to online matching,

Despite the fact that our model is inspired by online bipartite matching, it also overlaps with stochastic online scheduling problems (\sos)~\cite{megow2004stochastic,megow2006models,skutella2016unrelated}. We first restate our model 
in the language of \sos: we have $|U|$ {\it nonidentical } parallel machines and $|V|$ jobs; at every time-step a single job $v$ is sampled from $V$ with probability $p_{v,t}$; the jobs have to be assigned immediately after its arrival; additionally each job $v$ can be processed {\it non-preemptively} on a specific subset of machines; once we assign $v$ to $u$, we get a profit of $w_e$ and $u$ will be occupied for $C_e$ rounds with $e=(u,v)$, where $C_e$ is a random variable with known distribution. Observe that the key difference between our model and \sos is in the objective: the former is to maximize the expected profit from the completed jobs, while the latter is to minimize the total or the maximum completion time of all jobs.

\begin{comment}
Another notable issue is the interesting link between the offline version of our model and stochastic knapsack problem~\cite{dean2005adaptivity, gupta2011approximation, ma2014improvements}. Consider the simple case when $|U|=1$. The offline version of our model can be stated in the language of stochastic knapsack problem as follows: we have a budget $T$ and $T$ items, say $(v_1, \ldots, v_T)$; each item $v$ has a stochastic integral size $C_e \in \{0,1,\ldots, T\}$ with $e=(u,v)$ with a known distribution; we obtain a profit of $w_e$ with $e=(u,v)$ once we successfully insert $v$ into the knapsack (\ie the size does not cause overflow); the goal is to design an efficient (offline) policy such that the expected total weight of all items inserted is maximized. Observe that the only extra restriction here is the time: we can process each item $v_t$ no earlier than $t$. 
\end{comment}






	


==> 5_hardness.tex <==
\section{Hardness Result}
\label{sec:hard}

%{\color{blue} state in introduction that by default we assume $|V|$ and $T$ are sufficiently large.}

Consider a complete bipartite graph of $G=(U,V,E)$ where $|U|=K$, $|V|=n^2$. Suppose we have $T=n$ rounds and $p_{v,t}=\frac{1}{n^2}$ for each $v$ and $t$. In other words, in each round $t$, each $v$ is sampled uniformly from $V$. For each $e$, let $C_e$ be a constant of $K$, which implies that each $u$ will be unavailable for a constant $K$ rounds after each assignment. Assume all assignments have a uniform weight (\ie $w_e=1$ for all $e$). Split the whole online process of $n$ rounds into $n-K+1$ consecutive windows $\cW=\{W_\ell\}$ such that $W_\ell=\{\ell, \ell+1, \ldots, \ell+K-1\}$ for each $1 \le \ell \le n-K+1$. The benchmark LP~\eqref{LP:offline-a} then reduces to the following.


\vspace*{-0.1in}
\begin{alignat}{2}
\label{LP:offline-b}
\text{max}    &  \sum_{t\in [T]} \sum_{e \in E} x_{e,t}   \\
\text{s.t.}  &  \sum_{e \in \nr{v} } x_{e,t} \le  \frac{1}{n^2}     & \ & \quad\forall v \in V, t\in [T] \label{cons:vb}\\
                   & \sum_{t \in W_\ell} \sum_{e \in \nr{u} }x_{e,t}       \le 1    &\ & \quad\forall u \in U, 1\le \ell  \le n-K+1 \label{cons:ub}\\
                   & 0 \le x_{e,t} \le 1                   &\ & \quad\forall e \in E, t\in [T] \label{LP:offline-end-b}
\end{alignat}
 
We can verify that an optimal solution to the above LP is as follows: $x^*_{e,t}= 1/(n^2K)$ for all $e$ and $t$ with the optimal objective value of $n$. We investigate the performance of any optimal non-adaptive algorithm. Notice that the expected arrivals of any $v$ in the full sequence of online arrivals is $1/n$. Thus for any non-adaptive algorithm $\NALG$,  it needs to specify the allocation distribution $\cD_v$ for each $v$ during the first arrival. Consider a given $\NALG$ parameterized by $\{\alpha_{u,v} \in [0,1]\}$ for each $v$ and $u \in \nr{v}$ such that $\sum_{u \in \nr{v}} \alpha_{u,v} \le 1$ for each $v$. In other words, $\NALG$ will assign $v$ to $u$ with probability $\alpha_{u,v}$ when $v$ comes for the first time and $u$ is available. 

Let $\beta_u=\sum_{v \in \nr{u}} \alpha_{u,v}*\frac{1}{n^2}$, which is the probability that $u$ is matched in each round if it is safe at the beginning of that round, when running $\NALG$. Hence, 
\begin{equation*}\label{eqn:hard-1}
\sum_{u \in U} \beta_u = \sum_{u \in U}\sum_{v \in \nr{u}} \alpha_{u,v}*\frac{1}{n^2} =
\sum_{v \in V}\sum_{u \in \nr{v}} \alpha_{u,v}*\frac{1}{n^2} \le 1
\end{equation*}

Consider a given $u$ with $\beta_u$ and let $\gamma_{u,t}$ be the probability that $u$ is available at $t$. Then the expected number of matches of $u$ after the $n$ rounds is $\sum_t \beta_u \gamma_{u,t}$. We have the recursive inequalities on $\gamma_{u,t}$ as in Lemma~\ref{eqn:hard-2}, with $\gamma_{u,t}=1, t=1$.

\begin{lemma}
\label{eqn:hard-2}
$\forall 1<t \le n$, we have	
\[ \gamma_{u,t}+\beta_{u} \sum_{ t-K+1 \le t' <t } \gamma_{u,t'} = 1 \]
\end{lemma}

Note that the \OPT of our benchmark LP is $n$ while the performance of $\NALG$ is $\sum_u \sum_t \beta_u \gamma_{u,t}$. The resulting competitive ratio achieved by an optimal \NALG is captured by the following maximization program.


\begin{equation}\label{eqn:hard-3}
\resizebox{0.91\hsize}{!}{
$
\begin{aligned}
&{\text{max}}
&&\frac{\sum_u  \sum_t \beta_u \gamma_{u,t}}{n} \\
&\text{s.t.} 
&&  \sum_{u \in U} \beta_{u}  \le 1 & \\
&&&\gamma_{u,t}+\beta_{u} \sum_{ t-K+1 \le t' <t } \gamma_{u,t'} = 1
& \forall  1<t\le n, u \in U\\
&&& \beta_u \ge 0, \gamma_{u, 1}=1  & \forall u \in U
\end{aligned}
$
}
\end{equation}

We prove the following Lemma which implies Theorem~\ref{thm:2}.

\begin{lemma}\label{lem:hard-3}
The optimal value to the program~\eqref{eqn:hard-3} is at most $\frac{1}{2-1/K}+o(1)$ when $K=o(n)$. 
\end{lemma}

 %A detailed proof is omitted here. 
\begin{comment}
\begin{proof}
Focus on a given $u$. Notice that $\gamma_{u,t}+\beta_{u} \sum_{ t-K+1 \le t' <t } \gamma_{u,t'} = 1$ for all $1 \le t\le n$. Sum all equations over $t \in [n]$, we have
\begin{eqnarray*}
 \Big(1+\beta_u(K-1)\Big) \sum_{t \in [n]} \gamma_{u,t}&=& n+\beta_u(K-1)\gamma_{u,n}+\beta_u(K-2)\gamma_{u,n-1}+\cdots+ \beta_u\gamma_{u, n-K+2}\\
 & \le &  n+K-1
\end{eqnarray*}
Therefore we have 
$$\sum_{t\in [n]} \gamma_{u,t} \le \frac{n}{1+\beta_u(K-1)}+\frac{K-1}{1+\beta_u(K-1)} \le \frac{n}{1+\beta_u(K-1)}+\frac{1}{\beta_u}$$

Define $H_u \doteq  \sum_t \beta_u \gamma_{u,t}$. From the above analysis, we have
$H_u \le  \frac{n \beta_u}{1+\beta_u(K-1)}+1$. Thus the objective value in the program~\eqref{eqn:hard-3} should be at most
$$ \frac{\sum_u  \sum_t \beta_u \gamma_{u,t}}{n} =\sum_{u \in U} \frac{H_u}{n}
\le \sum_{u\in U}  \frac{ \beta_u}{1+\beta_u(K-1)}+\frac{K}{n}$$

We claim that the optimal value to the program~\eqref{eqn:hard-3} can be upper bounded by the below maximization program:
$$\left\{  \max \sum_{u\in[U]} \frac{\beta_u}{1+\beta_u(K-1)} +\frac{K}{n}:~~ \sum_{u\in U} \beta_u=1, \beta_u \ge 0,\forall u \in U \right\}$$

According to our assumption $K=o(n)$, the second term can be ignored. Let $g(x)=x/(1+x (K-1))$. For any $K \ge 2$, it is a concave function, which implies that maximization of $g$ subject to $\sum_u \beta_u=1$ will be achieved when all $\beta_u=1/K$. The resultant value is $\frac{1}{2-1/K}+o(1)$. Thus we are done.
\end{proof}
\end{comment}


\xhdr{Unconditional Hardness.} \citet{manshadi2012online} prove that for the online matching problem under known distribution (but disposable offline vertices), no algorithm can achieve a ratio better than $0.823$. Since, our setting generalizes this, the hardness results directly apply to our problem as well.

%$\{\cD_v \}$ such that $\cD_v=\{ \alpha_{u,v}| u \in \nr{v}\}$ for each $v$, where  
% \ie $\Pr[C_e=K]=1$
%from a known identical independent distributions (IID) 





==> 5_main_alg.tex <==


\section{Simulation-based Algorithm}
\label{sec_main_alg}
		%We present a simulation-based adaptive algorithm. 
		 In this section, we present a simulation-based algorithm. Proofs for Lemma~\ref{lem:sim}, \ref{eqn:hard-2} and \ref{lem:hard-3} can be found in the supplementary material. The main idea is as follows. Let $\vec{x}^*$ denote an optimal solution to LP~\eqref{LP:offline-a}. Suppose we aim to develop an online algorithm achieving a ratio of $\gamma \in [0,1]$. Consider an assignment $e=(u,v)$ when some $v$ arrived at time $t$. Let $\SF_{e,t}$ be the event that $e$ is safe at $t$, \ie $u$ is available at $t$. By simulating the current strategy up to $t$, we can get an estimation of $\Pr[\SF_{e,t}]$, say $\beta_{e,t}$, within an arbitrary small error. Therefore in the case $e$ is safe at $t$, we can sample it with probability $\frac{x^*_{e,t}}{p_{v,t}}\frac{\gamma}{\beta_{e,t}}$, which leads to the fact that $e$ is sampled with probability $\gamma x^*_{e,t}$ unconditionally. Hence, we call any algorithm that satisfies $\gamma \leq \beta_{e, t}$ as \emph{valid}.
 
 The simulation-based attenuation technique has been used previously for other problems, such as stochastic knapsack~\cite{ma2014improvements} and stochastic matching~\cite{adamczyk2015improved}. Throughout the analysis, we assume that we know the exact value of $\beta_{e,t} := \Pr[\SF_{e,t}]$ for all $t$ and $e$. (It is easy to see that the sampling error can be folded into a multiplicative factor of $(1 - \epsilon)$ in the competitive ratio by standard Chernoff bounds and hence, ignoring it leads to a cleaner presentation). The formal statement of our algorithm, denoted by $\adap(\gamma)$, is as follows. For each $v$ and $t$, let $\nr{v,t}$ be the set of {\it safe} assignments for $v$ at  $t$.
 
 %available neighbors of $v$ at $t$ and $\cN_v$ be the set of neighbors of $v$ initially. 

		
  \begin{algorithm}[h]
\label{alg:adap}
\caption{Simulation-based adaptive algorithm ($\adap (\gamma))$} 
\DontPrintSemicolon
For each time $t$, let $v$ denote the request arriving at time $t$.\;
If $\nr{v,t}=\emptyset$, then reject $v$; otherwise choose $e \in \nr{v,t}$ with prob. $\frac{x^*_{e,t}}{p_{v,t}}\frac{\gamma}{\beta_{e,t}}$ where $e=(u,v)$.
\end{algorithm}


\begin{lemma}\label{lem:sim}
$\adap(\gamma)$ is valid with $\gamma=\frac{1}{2}$.
\end{lemma}

The main Theorem~\ref{thm:1} follows directly from Lemmas~\ref{lem:lp} and~\ref{lem:sim}.

\xhdr{Extension from $C_e$ to $C_{e,t}$.} Consider the case when the occupation time of $u$ from $e$ is sensitive to $t$. In other words, each $u$ will be unavailable for $C_{e,t}$ rounds from the assignment $e=(u,v)$ at $t$. We can accommodate the extension by simply updating the constraints~\eqref{cons:u} on $u$ in the benchmark LP~\eqref{LP:offline-a} to the following. We have that $\forall u \in U, t \in [T]$,

\begin{equation}\label{cons:new_u}
\sum_{t'<t} \sum_{e \in \nr{u} }x_{e,t'} \Pr[C_{e,t'}>t-t'] +\sum_{e \in \nr{u}} x_{e,t}  \le 1   
\end{equation}
The rest of our algorithm remains the same as before. We can verify that (1) LP~\eqref{LP:offline-a} with constraints~\eqref{cons:u} replaced by~\eqref{cons:new_u} is a valid benchmark; (2) $\adap$ achieves a competitive ratio of $\frac{1}{2}-\epsilon$ for any given $\epsilon>0$ for the new model based on the new valid benchmark LP. The modifications to the analysis transfer through in a straightforward way and for brevity we omit the details here. 













 


==> 5_main_model.tex <==
\section{Main Model}
\label{sec:main-model}
In this section, we present a formal statement of our main model. Suppose we have a bipartite graph $G=(U,V, E)$ where $U$ and $V$ represent offline and online parties respectively. 
 We have a finite time horizon $T$ (known beforehand) and for each time $t \in [T]$, a vertex $v$ will be sampled (we use the term $v$ \emph{arrives}) from a known probability distribution $\{p_{v,t}\}$ such that $\sum_{v \in V} p_{v,t} \le 1$\footnote{Thus, with probability $1-\sum_{v \in V} p_{v,t}$, none of the vertices from $V$ will arrive at $t$.} (noting that such a choice is made independently for each round $t$). The expected number of times $v$ arrives across the $T$ rounds, $\sum_{t \in [T]} p_{v, t}$ is called the \emph{arrival rate} for vertex $v$. Once a vertex $v$ arrives, we need to make an {\it irrevocable decision immediately}: either to reject $v$ or assign $v$ to one of its neighbors in $U$. For each $u$, once it is assigned to some $v$, it becomes unavailable for $\re_e$ rounds with $e=(u,v)$, and subsequently rejoins the system. 
Here $\re_e$ is an integral random variable taking values from $\{0,1,\ldots,T\}$ and the distribution is known in advance. Each assignment $e$ is associated with a weight $w_e$ and our goal is to design an online assignment policy such that the total expected weights of all assignments made is maximized. Following prior work, we assume $|V| \gg |U|$ and $T\gg 1$. Throughout this paper, we use edge $e=(u,v)$ and assignment of $v$ to $u$ interchangeably. 

For an assignment $e$, let $x_{e,t}$ be the probability that $e$ is chosen at $t$ in any offline optimal algorithm. For each $u$ (likewise for $v$), let $\nr{u}$ ($\nr{v}$) be the set of neighboring edges incident to $u$ ($v$). We use the LP \eqref{LP:offline-a} as a benchmark to upper bound the offline optimal. We now interpret the constraints. For each round $t$, once an online vertex $v$ arrives, we can assign it to at most one of its neighbors. Thus, we have: if $v$ arrives at $t$, the total number of assignments for $v$ at $t$ is at most 1; if $v$ does not arrive, the total is 0. The LHS  of \eqref{cons:v} is exactly the expected number of assignments made at $t$ for $v$. It should be no more than the prob. that $v$ arrives at $t$, which is the RHS of \eqref{cons:v}. Constraint \eqref{cons:u} is the \emph{most} novel part of our problem formulation. Consider a given $u$ and $t$. In the LHS, the first term (summation over $t' < t$ and $e \in \nr{u}$) refers to the prob. that $u$ is not available at $t$ while the second term (summation over $e \in \nr{u}$) is the prob. that $u$ is assigned to some worker at $t$, which is no larger than prob. $u$ is available at $t$. Thus, the sum of the first term and second term on LHS is no larger than 1.\footnote{We would like to point out that our LP constraint~\eqref{cons:u} on $u$ is inspired by~\citet{ma2014improvements}. The proof is similar to that by~\citet{alaei2012online} and~\citet{alaei2013online}. 
} This argument implies that the \LP forms a valid upper-bound on the offline optimal solution and hence we have Lemma~\ref{lem:lp}.

\begin{figure*}{!h}
\begin{alignat}{2}
\label{LP:offline-a}
\text{maximize}    &  \sum_{t\in [T]} \sum_{e \in E} w_{e}x_{e,t}  & \\
\text{subject to}  &  \sum_{e \in \nr{v} } x_{e,t} \le  p_{v,t}     &  \qquad \forall v \in V, t\in [T] \label{cons:v}\\
                   & \sum_{t'<t} \sum_{e \in \nr{u} }x_{e,t'} \Pr[C_e>t-t'] +\sum_{e \in \nr{u}} x_{e,t}        \le 1    & \qquad \forall u \in U, t \in [T]\label{cons:u}\\
                   & 0 \le x_{e,t} \le 1   & \forall e \in E, t\in [T] \label{LP:offline-d}
\end{alignat}
\end{figure*}

 
\begin{lemma}\label{lem:lp}
The optimal value to LP \eqref{LP:offline-a} is a valid upper bound for the offline optimal. 
\end{lemma}

%\footnote{}
%\begin{comment}
%\begin{proof}
%Notice that $\sum_{e \in E_v} x_{e,t}$ is the expected number of assignments made with respect to $v$ at $t$, which should be no  larger than the probability that $v$ arrives at $t$. Thus constraints~\eqref{cons:v} on $v$ are valid.
%
%As for constraints~\eqref{cons:u} on $u$: note that the first term of $\sum_{t'<t} \sum_{e \in \nr{u} }x_{e,t'} \Pr[C_e>t-t']$ is exactly the probability that $u$ is not available at $t$ and the second term of $\sum_{e \in \nr{u}} x_{e,t} $ is the probability that one assignment is made at $t$ with respect to $u$. Therefore the sum should be at most $1$.
%\end{proof}
%\end{comment}





% \footnote{We will consider a slightly more general setting of $\re_{e,t}$ later where the }
%Let $\la=(u,v,t)$ denote an assignment of $v$ to $u$ at $t$. For a $\la=(u,v,t)$, we use $\la_1, \la_2$ and $\la_3$ to refer the three components in $\la$, which are $u$, $v$ and $t$ respectively. Also we assume the weight of $\la=(u,v,t)$ is $w_\la=w_e$ with $e=(u,v)$.
%Let $x_{\la}$ be the probability that assignment $\la$ is made (\ie $e=(u,v)$ is made at $t$) in any offline optimal. We use the below LP as a benchmark to upper bound the offline optimal. 

%\begin{algorithm}[!h]
%\caption{$\HM(\alpha)$}
%\label{alg:hm-basic}
%\DontPrintSemicolon
%Initialize \cR to be the empty set. We will add edges to this set during the course of the algorithm and at the end will denote our returned set of matching. \;
%For each $e \in \cE$, generate an independent Bernoulli random variable $Y_{e}$ with mean $\alpha x_e$. \;
%Choose a random permutation $\pi$ over $\cE$ and follow $\pi$ to check each edge one by one: add $e$ to \cR if $Y_{e}=1$ and $e$ is safe, i.e., none of the vertices in $e$ are matched; otherwise skip it. \;			
%Return \cR as the matching. \;
%\end{algorithm}






==> 6_experiments.tex <==
%!TEX root = 0-17-NIPS.tex

\section{Experiments}
\label{sec:experiments}
		\begin{figure*}[!ht]
					\minipage{0.32\textwidth}
					\includegraphics[width=\linewidth]{normal_uniform.png}
					\caption{OTD is normal distribution under KIID}
					\label{fig:normaluniform}
					\endminipage\hfill
					\minipage{0.32\textwidth}
					\includegraphics[width=\linewidth]{normal_pjt.png}
					\caption{OTD is normal distribution under KAD}\label{fig:normal_pjt}
					\endminipage\hfill
					\minipage{0.32\textwidth}%
					\includegraphics[width=\linewidth]{powerlaw_pjt.png}
					\caption{OTD is power law distribution under KAD}\label{fig:powerlaw_pjt}
					\endminipage
				\end{figure*}
			
			
				\begin{figure*}[!ht]
					\minipage{0.32\textwidth}
					\includegraphics[width=\linewidth]{type_requests.png}
					\caption{The number of requests of a given type at various time-steps.  x-axis: time-step, y-aixs: number of requests}
					\label{fig:typerequests}
					\endminipage\hfill
					\minipage{0.32\textwidth}
					\includegraphics[width=\linewidth]{reappeardistribution_figure.png}
					\caption{Occupation time distribution of all cars. x-axis: number of time-steps, y-axis: number of requests }\label{fig:reappearDistributionAll}
					\endminipage\hfill
					\minipage{0.32\textwidth}%
					\includegraphics[width=\linewidth]{two_specific_reappeardistribution_figure.png}
					\caption{Occupation time distribution of two different cars. x-axis: number of time-steps, y-axis: number of requests}\label{fig:tworeappear}
					\endminipage
				\end{figure*}


%	In this section, we summarize our discussion on the preliminary experimental results. We implemented our matching algorithms and tested them on a ride-sharing dataset. We also provide a few heuristics which have good performance on this dataset. We provide a discussion justifying the model assumptions, algorithm and implications.
	\label{sec:experiments-dataset}
To validate the approaches presented in this paper, we use the New York City yellow cabs dataset,\footnote{\texttt{http://www.andresmh.com/nyctaxitrips/}} which contains the trip records for trips in Manhattan, Brooklyn, and Queens for the year $2013$. The dataset is split into $12$ months. For each month we have numerous records each corresponding to a single trip. Each record has the following structure. We have an anonymized license number which is the primary key corresponding to a car. For privacy purposes a long string is used as opposed to the actual license number. We then have the time at which the trip was initiated, the time at which the trip ended, and the total time of the trip in seconds. This is followed by the starting coordinates (\ie latitude and longitude) of the trip and the destination coordinates of the trip.
			%\vspace{-1mm}
			
			\xhdr{Assumptions.} We make two assumptions specific to our experimental setup. Firstly, we assume that every \emph{car} starts and ends at the same location, for \emph{all} trips that it makes. Initially, we assign every car a location (potentially the same) which corresponds to its \emph{docking} position. On receiving a request, the car leaves from this docking position to the point of pick-up, executes the trip and returns to this docking position. Secondly, we assume that occupation time distributions (OTD) associated with all matches are identically (and independently) distributed, \ie $\{\re_e\}$ follow the same distribution. Note that this is a much stronger assumption than what we made in the model, and is completely inspired by the dataset (see Section~\ref{sec:exp_ana}). We test our model on two specific distributions, namely a \emph{normal} distribution and the \emph{power-law} distribution (see Figure~\ref{fig:reappearDistributionAll}). The docking position of each car and parameters associated with each distribution are all learned from the training dataset (described below in the {\bf Training} discussion).
			
		
			%			of all cars follows the same distribution, \ie $\{\re_e |e \in E\}$ are all identically (and independently) distributed.
			%We learn the parameters of the normal distribution (\ie the mean and standard deviation) and power law distribution (\ie the constant and the exponent) from the training set. We infer this docking position from our training data.
			
	

		
		\subsection{Experimental Setup}
			For our experimental setup, we randomly select $30$ cabs (each cab is denoted by $u$). We discretize the Manhattan map into cells such that each cell is approximately $4$ miles (increments of $0.15$ degrees in latitude and longitude). For each pair of locations, say $(a,b)$, we create a request \emph{type} $v$, which represents all trips with starting and ending locations falling into $a$ and $b$ respectively. In our model, we have
		$|U|=30$ and $|V| \approx 550$ (variations depending on day to day requests with low variance).
			 We focus on the month of January $2013$. We split the records into $31$ parts, each corresponding to a day of January. We choose a random set of $12$ parts for \emph{training} purposes and use the remaining for \emph{testing} purposes. 

The edge weight $w_e$ on $e=(u,v)$ (\ie edge from a car $u$ to type $v$) is set as a function of two distances in our setup. The first is the trip distance (\ie the distance from the starting location to the ending location of $v$, denoted $L_1$) while the second is the docking distance (\ie the distance from the docking position of $u$ to the starting/ending location of $v$, denoted $L_2$). We set $w_e=\max(L_1-\alpha L_2, 0)$, where $\alpha$ is a parameter capturing the subtle balance between the positive contribution from the trip distance and negative contribution from the docking distance to the final profit. We set $\alpha=0.5$ for the experiments. We consider each single day as the time horizon and set the total number of rounds $T=\frac{24*60}{5}=288$ by discretizing the $24$-hour period into a time-step of $5$ minutes. Throughout this section, we use time-step and round interchangeably. 

%When a request comes, the former remains same for all free vertices while the latter determines the differences in the edge-weights. In other words, weight = $L_1$ - $\alpha L_2$. Increasing $\alpha$ pronounces the difference between \LP based algorithms and uniform sampling while setting $\alpha=0$ would make these two algorithms coincide.


%Let $l(u)$, $s(v)$ and $e(v)$ denote the docking position of $u$, the starting and ending location of $v$ respectively. Set $L(v)=\dis(l_1(v), l_2(v))-\dis(l(u), l_1(v))-\dis(l(u),l_2(v))$.

			
%We assign every edge $(u, v)$ (\ie edge from a car $u$ to type $v$) a weight that is based on the distance between the docking position of $u$, the start and end location of type $v$. Let $r$ denote the trip-distance of $v$ minus the sum of distances between docking position of $u$ to starting position of $v$ and end position of $v$ to the docking position of $u$. If $r$ is non-negative, we assign the weight with $r$, else with a weight of $0$ (\ie no edge).
%			We would like to point out that the results in the experiments are sensitive to two key parameters. The first parameter is the discretization of the time-steps. In particular, we discretize the 24-hour period into steps of 5 minutes. We assume that all requests arriving within this five minute window corresponds to a single time-step in the algorithm. Hence, varying the size of this window leads to increased/decreased arrival rates, which in turn leads to variation in performance (\eg when the rates are very low, our algorithm approaches the worst-case ratio of 0.5). \kaedit{move this sentence to discussion.} The second parameter is edge-weights. Edge-weights are a function of two distances in our setup. The first is the trip-length (denote $L_1$) while the second is the distance from the docking position to start/end of the trip (denote $L_2$). When a request comes, the former remains same for all free vertices while the latter determines the differences in the edge-weights. In other words, weight = $L_1$ - $\alpha L_2$. Increasing $\alpha$ pronounces the difference between \LP based algorithms and uniform sampling while setting $\alpha=0$ would make these two algorithms coincide.
			\vspace{-1mm}
			\xhdr{Training.} We use the training dataset of $12$ days to learn various parameters. As for the arrival rates $\{p_{v,t}\}$, we count the total number of appearances of each request type $v$ at time-step $t$ in the $12$ parts (denote it by $c_{v,t}$) and set $p_{v,t}=c_{v,t}/12$ under KAD. When assuming KIID, we set  $p_v=p_{v,t}  = (c/12)/T$ (\ie the arrival distributions are assumed the same across all the time-steps for each $v$). The estimation of parameters for the two different occupation time distributions are processed as follows. We first compute the average number of seconds between two \emph{requests} in the dataset (note this was $5$ minutes in the experimental setup). We then assume that each \emph{time-step} of our online process corresponds to a time-difference of this average in seconds. We then compute the sample mean and sample variance of the trip lengths (as number of seconds taken by the trip divided by five minutes) in the $12$ parts. Hence we use the normal distribution obtained by this sample mean and standard deviation as the distribution with which a car is unavailable. 
We assign the docking position of each car to the location (in the discretized space) in which the majority of the requests were initiated (\ie starting location of a request) and matched to this car.
			
			%As for the docking position to each car, we 
			%we look at the requests that were matched to a particular car in the dataset. 
		%\subsection{Justification of Model Assumptions and Results}
			%	We will first describe some exploratory analysis on this dataset. This will help us validate our model assumptions and design and justify the experimental setup.
				
			%	 in two ways: (1) It will show the validity of our model specifications and (2) It will help us design and justify the experimental setup.
			\subsection{Justifying The Two Important Model Assumptions}
				\label{sec:exp_ana}
				\xhdr{Known Adversarial Distributions.} Figure~\ref{fig:typerequests} plots the number of arrivals of a particular type at various times during the day. Notice the significant increase in the number of requests in the middle of the day as opposed to the mornings and nights. This justified our arrival assumption of KAD which assumes different arrival distributions at different time-steps. Hence the \LP (and the corresponding algorithm) can exploit this vast difference in the arrival rates and potentially obtain improved results compared to the assumption of Known Identical Independent Distributions (KIID). This is confirmed by our experimental results shown in Figures~\ref{fig:normaluniform} and~\ref{fig:normal_pjt}.  
				
								
	%This is a key assumption made in our model, which assumes the arrival distribution changes during different time. 		 (see the results sub-section where we compare against using an uniform distribution at all time-steps.)
	

				%\vspace{-3mm}
				\xhdr{Identical Occupation Time Distribution.}  We assume each car will be available again via an independent and identical random process regardless of the matches it received. The validity of our assumptions can be seen in Figures~\ref{fig:reappearDistributionAll} and~\ref{fig:tworeappear}, where the $x$-axis represents the different occupation time and the $y$-axis represents the corresponding number of requests in the dataset responsible for each occupation time. It is clear that for most requests the occupation time is around 2-3 time-steps and dropping drastically beyond that with a long tail. Figure~\ref{fig:tworeappear} displays occupation times for two representative (we chose two out of the many cars we plotted, at random) cars in the dataset; we see that the distributions roughly coincide with each other, suggesting that such distributions can be learned from historical data and used as a guide for future matches. 
				%Finally, we would like to point out that for all cars, the actual shape of the distribution is very close with only difference being in amplitude and phase (see Figure~\ref{fig:tworeappear}).

				
	
								
			\subsection{Results}
			 Inspired by the experimental setup by \cite{tong2016online,tong2016online_icde}, we run five different algorithms on our dataset. The first algorithm is the $\ALG$-$\LP$. In this algorithm, when a request $v$ arrives, we choose a neighbor $u$ with probability $x^*_{e,t}/p_{v,t}$ with $e=(u,v)$ if $u$ is available. Here $x^*_{e,t}$ is an optimal solution to our benchmark \LP and $p_{v,t}$ is the arrival rate of type $v$ at time-step $t$. The second algorithm is called \sclp. Recall that $E_{v,t}$ is the set of ``safe"
or available assignments with respect to $v$ when the type $v$ arrives at $t$. Let $x_{v,t}= \sum_{e \in E_{v,t}} x^*_{e,t}$. In \sclp, we sample a safe assignment for $v$ with probability $x^*_{e,t}/x_{v,t}$. The next two algorithms are heuristics oblivious to the underlying $\LP$. Our third algorithm is called \greedy which is as follows. When a request $v$ comes, match it to the safe neighbor $u$ with the highest edge weight. Our fourth algorithm is called \uralg which chooses one of the safe neighbors uniformly at random. Finally, we use a combination of $\LP$-oblivious algorithm and $\LP$-based algorithm called \egreedy. In this algorithm when a type $v$ comes, with probability $\epsilon$ we use the greedy choice and with probability $1-\epsilon$ we use the optimal $\LP$ choice. In our algorithm, we optimized the value of $\epsilon$ and set it to $\epsilon = 0.1$. We summarize our results in the following plots. Figures~\ref{fig:normaluniform}, \ref{fig:normal_pjt}, and~\ref{fig:powerlaw_pjt} show the performance of the five algorithms and \OPT (optimal value of the benchmark \LP) under the different assumptions of the OTD (normal or power law) and online arrives (KIID or KAD). In all three figures the x-axis represents test data-set number and the y-axis represents average weight of matching.
				% (denoted by $C_e \sim \cN$)

						
		\OMIT{
			\begin{figure}[!htb]
				\minipage{0.32\textwidth}
				\includegraphics[width=\linewidth]{combined_pjt.png}
				\caption{Performance of ALG-LP under two }
				\label{fig:combined}
				\endminipage
			\end{figure}
		}
	
			\xhdr{Discussion.}
				From the figures, it is clear that both the \LP-based solutions, namely $\ALG$-$\LP$ and \sclp, do better than choosing a free neighbor uniformly at random. Additionally, with distributional assumptions the \LP-based solutions outperform greedy algorithm as well. We would like to draw attention to a few interesting details in these results. Firstly, compared to the \LP optimal solution, our \LP-based algorithms have a competitive ratio in the range of $0.5$ to $0.7$. We believe this is because of our experimental setup. In particular, we have that the rates are high ($>0.1$) only in a few time-steps while in all other time-steps the rates are very close to $0$. This means that it resembles the structure of the \emph{theoretical} worst case example we showed in Section~\ref{sec:hard}. In future experiments, running our algorithms during \emph{peak} periods (where the request rates are significantly larger than $0$) may show that competitive ratios in those cases approach $1$. Secondly, it is surprising that our algorithm is fairly robust to the \emph{actual} distributional assumption we made. In particular, from Figures~\ref{fig:normal_pjt} and~\ref{fig:powerlaw_pjt} it is clear that the difference between the assumption of normal distribution versus power-law distribution for the unavailability of cars is \emph{negligible}. This is important since it might not be easy to learn the \emph{exact} distribution in many cases (\eg cases where the sample complexity is high) and this shows that a close approximation will still be as good.
				
			
			


==> 7_future.tex <==
\section{Conclusion and Future Directions}
	In this work, we provide a model that captures the application of assignment in ride-sharing platforms. One key aspect in our model is to consider the \emph{reusable} aspect of the offline resources. This helps in modeling many other important applications where agents enter and leave the system \emph{multiple} times (\eg organ allocation, crowdsourcing markets \cite{ho2012online}, and so on). Our work opens several important research directions. The first direction is to generalize the online model to the \emph{batch} setting. In other words, in each round we assume multiple arrivals from $V$. This assumption is useful in crowdsourcing markets (for example) where multiple tasks---but not all---become available at some time. The second direction is to consider a Markov model on the driver starting position. In this work, we assumed that each driver returns to her docking position. However, in many ride-sharing systems, drivers start a new trip from the position of the last-drop off. This leads to a Markovian system on the offline types, as opposed to the assumed static types in the present work. Finally, pairing our current work with more applied stochastic optimization and reinforcement learning approaches would be of practical interest to policymakers running taxi and bikeshare services~\cite{Singhvi15:Predicting,OMahony15:Data,Lowalekar16:Online,Verma17:Augmenting,Ghosh17:Dynamic}.

